Ring artifacts correction in compressed sensing tomographic reconstruction

We present a novel approach to handle ring artifacts correction in compressed sensing tomographic reconstruction. The correction is part of the reconstruction process, which differs from classical sinogram pre-processing and image post-processing techniques. The principle of compressed sensing tomographic reconstruction is presented. Then, we show that the ring artifacts correction can be integrated in the reconstruction problem formalism. We provide numerical results for both simulated and real data. This technique is included in the PyHST2 code which is used at the European Synchrotron Radiation Facility for tomographic reconstruction.

==> biblio.tex <==
@article{michel11,
  author    = {Vincent Michel and
               Alexandre Gramfort and
               Ga{\"{e}}l Varoquaux and
               Evelyn Eger and
               Bertrand Thirion},
  title     = {Total variation regularization for fMRI-based prediction of behaviour},
  journal   = {CoRR},
  year      = {2011},
  volume    = {abs/1102.1101},
  url       = {http://arxiv.org/abs/1102.1101},
  timestamp = {Thu, 13 Nov 2014 09:27:11 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1102-1101},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
@article{beckteboulle,
 author = {Beck, Amir and Teboulle, Marc},
 title = {A Fast Iterative Shrinkage-Thresholding Algorithm for Linear Inverse Problems},
 journal = {SIAM J. Img. Sci.},
 issue_date = {January 2009},
 volume = {2},
 number = {1},
 month = mar,
 year = {2009},
 issn = {1936-4954},
 pages = {183--202},
 numpages = {20},
 url = {http://dx.doi.org/10.1137/080716542},
 doi = {10.1137/080716542},
 acmid = {1658364},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
}
